KernelBench: Can LLMs Write Efficient GPU Kernels?

Efficient GPU kernels are crucial for building performant machine learning architectures, but writing them is a time-consuming challenge that requires significant expertise; therefore, we explore using language models (LMs) to automate kernel generation. We introduce KernelBench, an open-source framework for evaluating LMs' ability to write fast and correct kernels on a suite of 250 carefully selected PyTorch ML workloads. KernelBench represents a real-world engineering environment and making progress on the introduced benchmark directly translates to faster practical kernels. We introduce a new evaluation metric fast_p, which measures the percentage of generated kernels that are functionally correct and offer a speedup greater than an adjustable threshold p over baseline. Our experiments across various state-of-the-art models and test-time methods show that frontier reasoning models perform the best out of the box but still fall short overall, matching the PyTorch baseline in less than 20% of the cases. While we show that results can improve by leveraging execution and profiling feedback during iterative refinement, KernelBench remains a challenging benchmark, with its difficulty increasing as we raise speedup threshold p.

==> tables/greedy.tex <==
% Greey baseline table
\begin{table}[h]
\centering
\setlength{\tabcolsep}{2pt} % default is about 6pt
\begin{tabular}{lccc|ccc}
    \toprule
    $\textbf{\fast{1}}$ over: & \multicolumn{3}{c}{PyTorch Eager} & \multicolumn{3}{c}{torch.compile} \\ 
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    KernelBench Level & 1 & 2 & 3 & 1 & 2 & 3 \\ 
    \midrule
    GPT-4o              & 4\%  & 5\%  & 0\%  & 18\% & 4\%  & \textbf{4\%} \\
    OpenAI o1           & \underline{10}\% & \underline{24}\% & \textbf{12\%} & 28\% & \underline{19}\% & \textbf{4\%} \\
    DeepSeek V3         & 6\%  & 4\%  & \underline{8}\%  & 20\% & 2\%  & \underline{2}\%  \\
    DeepSeek R1         & \textbf{12\%} & \textbf{36\%} & 2\% & \textbf{38\%} & \textbf{37\%} & \underline{2}\%  \\
    Claude 3.5 Sonnet   & \underline{10}\% & 7\%  & 2\%  & \underline{29}\% & 2\%  & \underline{2}\%  \\
    Llama 3.1-70B Inst. & 3\%  & 0\%  & 0\%  & 11\% & 0\%  & 0\%  \\
    Llama 3.1-405B Inst.& 3\%  & 0\%  & 2\%  & 16\% & 0\%  & 0\%  \\
    \bottomrule
\end{tabular}

\caption{\textbf{KernelBench is a challenging benchmark for current LMs}. Here we present \fast{1}, i.e. the percentage of problems where the model-generated kernel is faster than the PyTorch Eager and \texttt{torch.compile} baseline (default config) on NVIDIA L40S. The \texttt{torch.compile} baseline runtime is sometimes slower than Torch Eager -- this is due to reproducible runtime overhead (\textit{not compile time}) that could be significant for small kernels in Level 1. We focus on PyTorch Eager for the rest of our analysis, but we elaborate on other baselines in Appendix~\ref{appendix:eval-methods-and-baselines}.}
\label{table:greedy-baseline}
\end{table}

==> tables/hardware-prompt-delta.tex <==
% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|}
% \hline
% \multicolumn{4}{|c|}{\rule{0pt}{12pt}\textbf{With Specs of NVIDIA A100}} \\ \hline
% \textbf{Models} & \textbf{fast\_1} & \textbf{fast\_0} & \textbf{Speedup} \\ \hline
% Llama 3.1 70B       & +2               & +4               & N/A               \\ 
% Deepseek V3     & -3               & -4               & 1                \\ 
% OpenAI o1       & +7               & +10              & 1                \\ 
% Deepseek R1     & -7               & -20              & 1.07             \\ \hline
% \multicolumn{4}{|c|}{\rule{0pt}{12pt}\textbf{With Specs of NVIDIA H100}} \\ \hline
% \textbf{Models} & \textbf{fast\_1} & \textbf{fast\_0} & \textbf{Speedup} \\ \hline
% Llama 3.1 70B       & +2               & +3               & N/A               \\ 
% Deepseek V3     & -2               & -3               & 1                \\ 
% OpenAI o1       & 0                & +2               & 1.01             \\ 
% Deepseek R1     & -12              & -14              & 1.06             \\ \hline
% \end{tabular}
% \caption{\textbf{Effect of Providing Hardware Information on NVIDIA A100 and H100}. Differences in fast\_1, fast\_0, and speedup on KernelBench Level 2 for NVIDIA A100 and H100 when models are provided hardware information in-context. \todo{DOUBLE CHECK THESE SPEEDUP, analyze o1 runs}}
% \label{tab:hw-prompt}
% \end{table}

\begin{table}[h]
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{4}{|c|}{\rule{0pt}{12pt}\textbf{With Specs of NVIDIA A100}} \\ \hline
\textbf{Models} & \makecell{\textbf{Correct}\\\textbf{(fast\textsubscript{0})}} & \makecell{\textbf{Faster}\\\textbf{(fast\textsubscript{1})}} & \textbf{Speedup} \\ \hline
Llama 3.1 70B       & \textcolor{green}{+4}       & \textcolor{green}{+2}       & N/A               \\ 
DeepSeek V3         & \textcolor{red}{-4}         & \textcolor{red}{-3}         & 1                \\ 
OpenAI o1           & \textcolor{green}{+10}      & \textcolor{green}{+7}       & 1                \\ 
DeepSeek R1         & \textcolor{red}{-20}        & \textcolor{red}{-7}         & 1.07             \\ \hline
\multicolumn{4}{|c|}{\rule{0pt}{12pt}\textbf{With Specs of NVIDIA H100}} \\ \hline
\textbf{Models} & \makecell{\textbf{Correct}\\\textbf{(fast\textsubscript{0})}} & \makecell{\textbf{Faster}\\\textbf{(fast\textsubscript{1})}} & \textbf{Speedup} \\ \hline
Llama 3.1 70B       & \textcolor{green}{+3}       & \textcolor{green}{+2}       & N/A               \\ 
DeepSeek V3         & \textcolor{red}{-3}         & \textcolor{red}{-2}         & 1                \\ 
OpenAI o1           & \textcolor{green}{+2}       & \textcolor{green}{0}        & 1.01             \\ 
DeepSeek R1         & \textcolor{red}{-14}        & \textcolor{red}{-7}        & 1.06             \\ \hline
\end{tabular}
\caption{\textbf{Effect of Providing Hardware Information on NVIDIA A100 and H100}. Differences in Correct (fast\textsubscript{0}), Correct and Faster (fast\textsubscript{1}), and speedup on KernelBench Level 2 for NVIDIA A100 and H100 when models are provided hardware information in-context.}
\label{tab:hw-prompt}
\end{table}




% old table - with inst stats
% \begin{table}[h]
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \textbf{GPU} & \multicolumn{2}{c|}{\textbf{A100}} & \multicolumn{2}{c|}{\textbf{H100}} \\ \hline
% \textbf{Diff}       & \textbf{fast\_1} & \textbf{\# Inst} & \textbf{fast\_1} & \textbf{\#Inst} \\ \hline
% Llama 70B             & \textbf{+2}& -3& \textbf{TBD}& TBD                 \\ \hline
% Deepseek V3           & \textbf{-3}            & +24& \textbf{-2}& +23\\ \hline
% OpenAI o1             & \textbf{TBD}            & TBD& \textbf{TBD}            & -50                 \\ \hline
% Deepseek R1           & \textbf{-7}& +39& \textbf{-12}& +59\\ \hline
% \end{tabular}
% \caption{The effect of including hardware specifications in single-shot generation on the overall fast\_1 metric and the average number of hardware-specific instruction on Level 2. We show the difference between no hardware info and with hardware info. Evaluated for NVIDIA A100 and H100 platforms.}
% \label{tab:hw-prompt}
% \end{table}

==> tables/verifier_table.tex <==
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|}
\hline
Multi-Turn& Llama 3.1 70B& DeepSeek V3& & \\ 
 k = 10& & & Multi-Sampling Multi-Turn&\\ \hline
Last Turn G& & & & XX \\ 
Last Turn G& & XX  & XX & XX \\ 
Multi-Turn & XX & XX  & XX & XX \\
\hline
\end{tabular}
}
\caption{Improving correctness with test-time methods: We compare fast\_0 (\%), the percentage of problems that have at least one correct solution, under various sample budget. We compare repeated sampling and iterative refinement under the same sample budget  for Llama 3.1 70B and DeepSeek V3.} 
\label{tab:correctness-test-time}
\end{table}

\todo{SIMON grab number and fill this in }                         
